VIINTER: View Interpolation with Implicit Neural Representations of Images

We present VIINTER, a method for view interpolation by interpolating the implicit neural representation (INR) of the captured images. We leverage the learned code vector associated with each image and interpolate between these codes to achieve viewpoint transitions. We propose several techniques that significantly enhance the interpolation quality. VIINTER signifies a new way to achieve view interpolation without constructing 3D structure, estimating camera poses, or computing pixel correspondence. We validate the effectiveness of VIINTER on several multi-view scenes with different types of camera layout and scene composition. As the development of INR of images (as opposed to surface or volume) has centered around tasks like image fitting and super-resolution, with VIINTER, we show its capability for view interpolation and offer a promising outlook on using INR for image manipulation tasks.

==> fig_7.tex <==
\begin{figure*}[!ht]
    \FigSevenSubfigB{./figures/Holo/Maria/00.jpeg}%
    ~
    \FigSevenSubfigB{./figures/Holo/Maria/01.jpeg}%
    ~
    \FigSevenSubfigB{./figures/Holo/Maria/02.jpeg}%
    ~
    \FigSevenSubfigB{./figures/Holo/Maria/03.jpeg}%
    ~
    \FigSevenSubfigB{./figures/Holo/Maria/04.jpeg}%


    \FigSevenSubfigA{./figures/Holo/Shiba/00.jpeg}%
    ~
    \FigSevenSubfigA{./figures/Holo/Shiba/01.jpeg}%
    ~
    \FigSevenSubfigA{./figures/Holo/Shiba/02.jpeg}%
    ~
    \FigSevenSubfigA{./figures/Holo/Shiba/03.jpeg}%
    ~
    \FigSevenSubfigA{./figures/Holo/Shiba/04.jpeg}%

    \FigSevenSubfigCaption{$t=0$}%
    ~
    \FigSevenSubfigCaption{$t=0.25$}%
    ~
    \FigSevenSubfigCaption{$t=0.5$}%
    ~
    \FigSevenSubfigCaption{$t=0.75$}%
    ~
    \FigSevenSubfigCaption{$t=1$}%

	\caption{{\bf Unstructured Light Field Results.} We interpolate learned codes of views $i$ and $j$ as $(1 - t)\cdot z_{i} + t\cdot z_{j}$. The camera movement between the two known views includes rotation and translation. The interpolation through INR smoothly transforms the perspective, despite never having access to 3D structure or camera pose. Images are zoomed in for easier evaluations.}
	\label{fig:HoloMorph}
	%\vspace{-5pt}
\end{figure*}

